Towards Size-Independent Generalization Bounds for Deep Operator Nets

In recent times machine learning methods have made significant advances in becoming a useful tool for analyzing physical systems. A particularly active area in this theme has been "physics-informed machine learning" which focuses on using neural nets for numerically solving differential equations. In this work, we aim to advance the theory of measuring out-of-sample error while training DeepONets - which is among the most versatile ways to solve P.D.E systems in one-shot. Firstly, for a class of DeepONets, we prove a bound on their Rademacher complexity which does not explicitly scale with the width of the nets involved. Secondly, we use this to show how the Huber loss can be chosen so that for these DeepONet classes generalization error bounds can be obtained that have no explicit dependence on the size of the nets. The effective capacity measure for DeepONets that we thus derive is also shown to correlate with the behavior of generalization error in experiments.

==> Sections/Experiments.tex <==
\subsection{An Experimental Exploration of the Proven Rademacher Complexity Bound for DeepONets}\label{sec:experiments}


For our experiments we consider the following specification of the Burgers' P.D.E. with periodic boundary conditions, 
\begin{align*}
\frac{\partial s}{\partial t}+s\frac{\partial s}{\partial x} &=\kappa\frac{\partial^2 s}{\partial x^2}, \quad (x,t)\in [{- \pi, \pi}]\times[0,{\rm T}]\\
s(x-\pi,t) = s(x+\pi,t),~&s(x,0)=u(x)
\end{align*}
where, $\kappa >0$ denotes the fluid viscosity, $\ u(x)$ is a $2\pi$-periodic initial condition with zero mean i.e. $\int_{-\pi}^{\pi}u (x)dx=0$ and $\rho,{\rm T}\in{\mathbb R}$.

Hence it follows that the solution operator of Definition \ref{def:G} corresponding to the above maps the initial condition $u$ to the solution to the Burgers' P.D.E., $s$. Hence, we will approximate the implicit solution operator $({\cal G})$ with a DeepONet ($\tilde{{\cal G}}$) 
- which for this case would be a map as follows,
\begin{align*}
\R^m \times \R^2 \rightarrow \R, ~(\v,\y) \mapsto \tilde{\cal G}(\v,\y) := \sum_{k=1}^q {\cal N}_{\rm B,k}(\v)\cdot {\cal N}_{\rm T,k}(\y)
\end{align*}
where ${\cal N}_{\rm B}$ and ${\cal N}_{\rm T}$ are any two neural nets mapping $\R^m \rightarrow \R^q$ and $\R^2 \rightarrow \R^q$ respectively - the Branch net and the Trunk net.
In above, $q$, the common output dimension of the branch and the trunk net is a hyperparameter for the experiment. 

The data required to set up the training for the above map $\tilde{G}$ can be summarized as a $3-$tuple of tensors, \\
$(u_{\rm training}, \ y_{\rm training}, \ s_{\rm training})$ of dimensions and descriptions as given below. 

\begin{itemize}
\item $u_{\rm training}\in \R^{N_{\rm training} \times m}=$ evaluations of the $N_{\rm training}$ number of input functions at the $m$ sensors. We denote the $i^{th}$ row of the above as, $[{u}_i(x_1), {u}_i(x_2), \dots, { u}_i(x_{\rm m})] \ \forall i \in \{1,\ldots,N_{\rm training} \}$

\item $y_{\rm training} \in \R^{N_{\rm training} \times P_{\rm training} \times 2}= P_{\rm training}$ number of uniformly sampled collocation points in $\R^2$ corresponding to each of the $N_{\rm training}$ number of input functions. And $\forall {\rm i} \in \{1,\ldots,N_{\rm training} \}$,  we denote the sampled points as $\{ (x_{\rm i,j},t_{\rm i,j}) \mid j = 1,\ldots,P_{\rm training} \} \stackrel{\rm uniform}{\sim}  \left([{-\pi,\pi}]\times[0,T] \right )^{P_{\rm training}}$

\item $s_{\rm training}\in{\mathbb R}^{N_{\rm training} \times \ P_{\rm training}}=$ the value of the numerical solution of the P.D.E. at the respective collocation points. And the $(i,j)^{\rm th}-$entry of this would be denoted as $s_{\rm i}(x_{\rm i,j},t_{\rm i,j})$.
\end{itemize}

In terms of the above training data, the corresponding training loss (Definition \ref{def:donloss}) is, 


\begin{align}\label{eq:exploss}
{\cal L}_{\rm Training}(\theta)= \frac{1}{N_{\rm training}P_{\rm training}}\sum_{i=1}^{N_{\rm training}}\sum_{j=1}^{P_{\rm training}}\ell \left ( s_i(x_{\rm i,j},t_{\rm i,j}) -\sum_{k=1}^q{\cal N}_{\mathrm{B,k}}(u_i(x_1),u_i(x_2),\dots,u_i(x_m))\cdot{\cal N}_{\mathrm{T,k}}(x_{\rm i,j},t_{\rm i,j}) \right )
\end{align}

whereby in our experiments $\ell$ is either chosen as the $\ell_2$ loss or the Huber loss and $\theta$ denotes the vector of all trainable parameters over both the nets. Similarly as above the test loss ${\cal L}_{\rm Test}$ would be defined corresponding to a random sampling of $N_{\rm test}$ input functions and $P_{\rm test}$ points in the domain of the P.D.E. where the true solution is known corresponding to each of these test input functions. 


Further, for our experiments, we sampled the input functions $u_i$ by sampling functions of the form, \\ $u_i(x) = \sum^{N}_{n=1} c_n \sin((n+1)x)$, where the coefficients were sampled as, $\ c_n \sim \mathcal{N}(0, A^2)$, with $A$ and $N$ being arbitrarily chosen constants. This way of sampling ensures that the functions chosen are all $2\pi$-periodic and will have zero mean in the interval $[-\pi, \pi]$ - as required in our setup. 

In this section, we demonstrate our Rademacher complexity bound by training DeepONets on the above loss function and measuring the generalization gap of the trained DeepONet obtained and computing for this trained DeepONet an upperbound on the essential part of our Rademacher bound (i.e. $\frac{\C_{n,n-1}}{\sqrt{m}} \,\left(\prod_{j=2}^{n-1}\tilde{\C}_{-j,-j}\right)$ where $\tilde{\cal C}_{-k,-k}$ is as defined in equation \ref{eq:cup}). Then we vary the number of training data (i.e. $N_{\rm training} \times P_{\rm training}$) and show that the two numbers computed above are significantly correlated as this training hyperparameter is varied. We use branch and trunk nets each of which are of depth $3$ and width $100$. 

\begin{figure}[!h]
    \centering
    \begin{minipage}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Sections/images/huber_delta0.25_300_1500.png}
        \caption{$\delta$=$0.25$, correlation = $0.857$ }
        \label{fig:huber_delta0.25_300_1500}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Sections/images/huber_delta0.4_300_2000.png}
        \caption{$\delta$=$0.4$, correlation = $0.791$}
        \label{fig:huber_delta0.4_300_2000}
    \end{minipage}
    \caption{\small The above plot shows the behaviour of the measured generalization error with respect to $\frac{\C_{3,2} \, \tilde{\C}_{-2,-2}}{\sqrt{m}}$ for training DeepONets with empirical loss as given in equation \ref{eq:exploss}, specialized to the Huber loss (Definition~\ref{def:huber}) for the stated values of $\delta$ and for the branch and the trunk nets being of depth $3$. Each point is labelled by the number of training data used in that experiment.}
    \label{fig:plot_huber}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.5\textwidth]{Sections/images/l2_500_4000.png}
    \caption{\small The above plot shows the behaviour of the measured generalization error with respect to $\frac{\C_{3,2} \, \tilde{\C}_{-2,-2}}{\sqrt{m}}$ for training DeepONets with empirical loss as given in equation \ref{eq:exploss},specialized to the $\ell_2$ loss and for the branch and the trunk nets being of depth $3$. Each point is labelled by the number of training data used in that experiment.}
    \label{fig:l2_500_4000}
\end{figure}

The correlation plots shown in  Figures~\ref{fig:huber_delta0.25_300_1500} and \ref{fig:huber_delta0.4_300_2000}, correspond to training on the Huber loss function, with two different values of $\delta$ - and the left plot corresponding to the special value of $\delta = \frac{1}{4}$ where the size independent generalization bound in Theorem \ref{thm:genbound} clicks for this setup. 


In Figure~\ref{fig:l2_500_4000} we repeat the same experiments but for the $\ell_2$ loss function and show that the required correlation persists even this loss which is outside the scope of Theorem \ref{thm:genbound}.
